Constraining the fundamental parameters of the O-type binary CPD-41degr7733

Using a set of high-resolution spectra, we studied the physical and orbital properties of the O-type binary CPD-41 7733, located in the core of \ngc. We report the unambiguous detection of the secondary spectral signature and we derive the first SB2 orbital solution of the system. The period is 5.6815 +/- 0.0015 d and the orbit has no significant eccentricity. CPD-41 7733 probably consists of stars of spectral types O8.5 and B3. As for other objects in the cluster, we observe discrepant luminosity classifications while using spectroscopic or brightness criteria. Still, the present analysis suggests that both components display physical parameters close to those of typical O8.5 and B3 dwarfs. We also analyze the X-ray light curves and spectra obtained during six 30 ks XMM-Newton pointings spread over the 5.7 d period. We find no significant variability between the different pointings, nor within the individual observations. The CPD-41 7733 X-ray spectrum is well reproduced by a three-temperature thermal mekal model with temperatures of 0.3, 0.8 and 2.4 keV. No X-ray overluminosity, resulting e.g. from a possible wind interaction, is observed. The emission of CPD-41 7733 is thus very representative of typical O-type star X-ray emission.

==> response <==
Answer to referee's report.

Dear Dr Gies,

Please find here below answers to your comments and questions. 


> I was struck by the 
> narrowness of the spectral lines for both star, which presumably 
> means that they are slow rotators.  It would be interesting to 
> see if this slow rotation is consistent with orbital synchronous 
> rotation.  

We estimated a projected rotational velocity of 84km/s for the primary, slightly larger than the synchronous rotation (~75 km/s). This is now mentioned in Sect. 4.3  

> Finally, the authors might want to comment on the remarkably 
> high binary frequency among the massive stars in this cluster. 

A paper is in preparation revising the work done by Garcia and Mermilliod (2001). Our conclusion is that the minimal spectroscopic binary fraction is about 63% (Sana et al., proceeding of the JENAM 2005 ), thus much lower than the 79% suggested by Garcia and Mermilliod. Beyond their erroneous orbital solution (resulting from a mistake in some of the Julian date used, see e.g. our paper on HD 152219 or CPD-41 7742 -- but this does not affect the binary fraction), we could not found as any binaries as they did. Our results rest on a large FEROS data set on all the O-type star in the cluster and a review of the literature. We believe that their data set was actually of a too poor quality to definitely to address the binarity of the objects. Though it is still possible that NGC 6231 has a large binary fraction (~ 80%), there is at the time no evidence for it. Only 10 out of the 16 O/WR stars are definite spectroscopic binaries.  

We feel that it would be too long to discuss this issue in the present paper, especially since it is only dealing with one object (recognize as well as a binary by GM01) and not on the complete population.


> p7,par2,l4  Since the authors do not report on their observed 
> equivalent width data for the primary, it is hard to judge 
> the errors in their flux dilution argument.  

Table 5 now gives prim and sec. EWs measured on the ESO/MPG 2.2m data. 
Errors on the  flux dilution were derived accounting both of the errors on the measured EW (based on the complete data set, not only the 2.2m data) and of the dispersion of the EW of equivalent 'typical' O stars. 

> I think some caution 
> is in order since they are comparing the He line strengths of 
> a very young object to those for many other (and possibly more 
> evolved) O-stars in which the surface He abundance may be enriched. 

This is true, but it is unlikely that the all the comparison stars are biased, therefore this will be taken into account in the error bars associated with the mean EW of the reference O stars. 


> My impression from Fig. 3 is that the secondary lines are about 
> 10 times weaker than the primary lines, so if these lines have
> comparable strength in the individual spectra, then the magnitude 
> difference is about delta M_V = 2.5.
>  For temperatures of 
> 34000 and 20000 K for the primary and secondary, respectively, 
> the surface flux ratio near 4500 Angstroms is about 2.8.
> Consequently, since the observed flux ratio goes like the 
> product of the surface flux and radius squared, I would expect
> that the ratio of primary to secondary radius is about 1.9. 
> Thus, for a primary radius of 8.5 solar radii (expected for 
> a slightly evolved O8.5 star; see Martins et al. 2005, A&A, 
> 436, 1049; their Table 4), the secondary radius will be 
> about 4.5 solar radii, close to the expected value for a 
> main sequence star.  Therefore, I think it most likely that 
> the secondary is a B2-3 V type star (and not a giant). 

Actually, it all depends on the adopted luminosity ratio. If, as you did, we assume that the secondary is about 10 times weaker, we result with a secondary radius about 5Rsol,
The dilution argument is indeed rather approximate as testified by the large error bars obtained : the 1sigma uncertainties on R2 is about 2Rsol.  Therefore there is no real contradiction as a radius of 4.5 (typical of B3V) is at 2 sigma. It is true that this does not allow us to discriminate between both classes.
We have however updated the discussion to suggest a possible larger l1 value based on the comparison of typical O8.5 and B3 stars luminosities. The latter argument indeed point towards two main sequence stars.


> p8,par3,l3  I think that the position of the target in the 
> observed cluster color-magnitude diagram indicates that the 
> primary is only just leaving from the main sequence, so it 
> is not surprising that the primary will have properties 
> intermediate between those of a main sequence and giant star.

Agree.


> p3,par2,l6  O II 4276?  This appears much weaker than the 
> nearby C II 4267 feature.  See the B-star model spectra 
> by Gummersbach and Kaufer at:
> http://www.lsw.uni-heidelberg.de/cgi-bin/websynspec.cgi

You are right. It is the CII 4267 line.

> p4,par2,l7  Are the errors in the mean velocities in Table 1
> comparable to the r.m.s. errors of the fit in Tables 3 and 4?

They are a bit lower but of comparable magnitude.


> p4,par2,l13  It would be helpful to give an estimate of the 
> period error in Tables 3 and 4.

Done, although this is not really an error on the periodicity of the phenomenon, but rather a confidence limit of the models (these are definitely two different things). This was the reason why we did not consider including them in the table. This is now done and explained in the update version of the paper.


> p5,par4,l10  The $\gamma_1$ parameter in row 7 of Table 4 is 
> playing two roles: relative to the systemic velocity for 
> columns 2 and 3 and absolute in column 4.  I think most readers
> will find this confusing. 

We have homogenize the notations and added a short explanation. We hope this will help the reader 


> p6,par2,l7  Are the equivalent widths quoted relative to the 
> continuum of the composite spectrum (primary plus secondary)? 

yes, this is now explicitly mentioned

> p6,par2,l11  What are the errors associated with the equivalent 
> width measurements?  I find it surprising, for example, that 
> the He I 4471 line is weaker than He I 4387, which is never 
> seen in other B-star spectra.   

Errors are now quoted in Table 5. Regarding HeI4471, it could be securely deblended on only one spectrum (the secondary has to be red-shifted, otherwise it blends with the primary OII on the blue side of HeI4471) and, according to the method used (either a multi-gaussian fit -- not very well reproducing the global profile of the blend -- or a simple integration over the secondary profile, adopting the primary wing as continuum) values from 25 to 100mA are obtained which shows that the measurement is probably unreliable. However, we agree with your point that He I 4471 EW should be larger than He I 4387 EW, which readily exclude the results of the second method. 

> The ratio of the Si III to Mg II 
> lines is about the same as that for B2 V stars in the models 
> of Gummersbach and Kaufer. 

This is true, though unfortunately, the model grid is rather scarce. Because of the limited strength of CII4267 compared to HeI4387, we preferred a slightly larger spectral type. 

> p7,par3,l13  There are some missing steps here about the assumed 
> bolometric corrections applied to find the radii. 

The bolometric correction was taken from the same reference that the Teff scale. This is now explicitly mentioned in the text.


> p9,par4,l1  See the Martins et al. (2005) calibration.  They suggest 
> typical masses of 19 to 24 solar masses for main sequence and 
> giant O8.5 stars.  If so, then the orbital inclination may be close 
> to 70 degrees, where eclipses are a possibility. 

Right. I modified the paragraph to mention this possibility although our photometric data do not indicate this is the case.


> p9,par4,l9  Did the authors plot their photometric data versus the 
> new orbital phase? 

Yes, no result.

> 
> p9,par1,l1  The frequency quoted does not correspond to a 12 d 
> period. 

Thanks for pointing out this typo. The quoted frequency has been corrected.


> p10,par2,l1  How unusual is the presence of a higher energy component? 

According to a recent work (Sana et al 2006, MNRAS  372, 661), it is seen in about 25% of the O stars in NGC6231 and it seems unrelated to the presence of a PMS companion (physically or in the line of sight). This is now briefly discussed. 


> Table 5.  It would be helpful to also list the corresponding 
> equivalent widths for the primary in a three column table:
> line identification, primary EW, secondary EW. 
> Add a footnote that the measurements are referred to the 
> combined flux of the binary (if that is the case).

The Table as been updated accordingly.


Other comments/suggestions (mostly regarding the phrasing) were all included in the updated version. Table captions were reduced to a brief title and the information previously contained in these captions has been incorporated into the core of the paper.  Tables and references presentation has been updated to match the ApJ standards. Finally, a few other minor modifications  have been brought to the text here and there in order to ease the reading, but have no real impact on the paper shape.

Should you have any further questions/comments, please let us know.


Thanks a lot for your careful reading.

Hugues Sana


> 
-- 
-----------------------------------------------------
            Hugues Sana
            European Southern Observatory
    +       Alonso de Cordova 3107 - Vitacura
 + E S +    Casilla 19001 - Santiago 19 - Chile
    O       Tel: (00 56) 2 463 3050
    +       Fax: (00 56) 2 463 3001  
            Email (prof.): hsana@eso.org       
            Email (private): hugues_sana@yahoo.fr   
-----------------------------------------------------


